GeRM: A Generalist Robotic Model with Mixture-of-experts for Quadruped Robot

Multi-task robot learning holds significant importance in tackling diverse and complex scenarios. However, current approaches are hindered by performance issues and difficulties in collecting training datasets. In this paper, we propose GeRM (Generalist Robotic Model). We utilize offline reinforcement learning to optimize data utilization strategies to learn from both demonstrations and sub-optimal data, thus surpassing the limitations of human demonstrations. Thereafter, we employ a transformer-based VLA network to process multi-modal inputs and output actions. By introducing the Mixture-of-Experts structure, GeRM allows faster inference speed with higher whole model capacity, and thus resolves the issue of limited RL parameters, enhancing model performance in multi-task learning while controlling computational costs. Through a series of experiments, we demonstrate that GeRM outperforms other methods across all tasks, while also validating its efficiency in both training and inference processes. Additionally, we uncover its potential to acquire emergent skills. Additionally, we contribute the QUARD-Auto dataset, collected automatically to support our training approach and foster advancements in multi-task quadruped robot learning. This work presents a new paradigm for reducing the cost of collecting robot data and driving progress in the multi-task learning community. You can reach our project and video through the link: https://songwxuan.github.io/GeRM/ .

==> tabletex/tab2_task_num.tex <==
\begin{table*}[t!]
 \vspace{-1.em}
\caption{
\textbf{Illustration of seen tasks.} ``Average Trajectory Length" represents the average length of the image-based trajectories used in all simulation data for each task. In this context, an image is collected by 10-step data collection method. The term ``Episode" signifies the number of experiments conducted for each task, which also corresponds to the number of trajectories. The mean trajectory length of each subtask is captured by the term ``Trajectory Length". The ``Example Instruction" describes different task scenarios, including various higher-level variables associated with the simulation.  
}
\label{tab:seentasks}
\vspace{-0.6em}
\renewcommand\arraystretch{1.1}% 行距
\scriptsize
\centering
%cell大小
% \setlength{\aboverulesep}{1.85mm}
% \setlength{\belowrulesep}{-0.05mm}
\setlength{\tabcolsep}{0.78mm}{
\begin{tabular}{p{0.22\columnwidth}p{0.15\columnwidth}p{0.7\columnwidth}p{0.7\columnwidth}} 
\hline
\textbf{Skill} & \textbf{Condition} & \textbf{Episode} \\
\hline
Go to \textit{Object} & Success & 72K\\
Go to \textit{Object} & Failure & 72K\\
Go to \textit{Object} and avoid the obstacle & Success & 63K\\
Go to \textit{Object} and avoid the obstacle & Failure & 63K\\
Stop \textit{Object} & Success & 89K\\
Stop \textit{Object} & Failure & 89K\\
Distinguish \textit{Letter}) & Success & 10K\\
Distinguish \textit{Letter}) & Failure & 10K\\
Go through \textit{Tunnel} & Success & 48K\\
Go through \textit{Tunnel} & Failure & 48K\\

\hline
Total    & 348K & The total number of episodes & \\

\hline

\end{tabular}
}
\vspace{-1.em}
\end{table*}
